Tunable viscous layers in Corbino geometry using density junctions

In sufficiently clean materials where electron-electron interactions are strong compared to momentum-relaxing scattering processes, electron transport resembles the flow of a viscous fluid. We study hydrodynamic electron transport across density interfaces (n-n junctions) in a 2DEG in the Corbino geometry. From numerical simulations in COMSOL using realistic parameters, we show that we can produce tunable viscous layers at the density interface by varying the density ratio of charge carriers. We quantitatively explain this observation with simple analytic expressions together with boundary conditions at the interface. We also show signatures of these viscous layers in the magnetoresistance. Breaking down viscous and ohmic contributions, we find that when outer radial region of the Corbino has higher charge density compared to the inner region, the viscous layers at the interface serve to suppress the magneto-resistance produced by momentum-relaxing scattering. Conversely, the magneto-resistance is enhanced when the inner region has higher density than the outer. Our results add to the repertoire of techniques for engineering viscous electron flows, which hold a promise for applications in future electronic devices.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
